Integrated Reasoning Engine for Pointer-related Code Clone Detection

Detecting similar code fragments, usually referred to as code clones, is an important task. In particular, code clone detection can have significant uses in the context of vulnerability discovery, refactoring and plagiarism detection. However, false positives are inevitable and always require manual reviews. In this paper, we propose Twin-Finder+, a novel closed-loop approach for pointer-related code clone detection that integrates machine learning and symbolic execution techniques to achieve precision. Twin-Finder+ introduces a formal verification mechanism to automate such manual reviews process. Our experimental results show Twin-Finder+ that can remove 91.69% false positives in average. We further conduct security analysis for memory safety using real-world applications, Links version 2.14 and libreOffice-6.0.0.1. Twin-Finder+ is able to find 6 unreported bugs in Links version 2.14 and one public patched bug in libreOffice-6.0.0.1.

==> Abstract.tex <==
\section*{Abstract}
Detecting code clones is crucial in various software engineering tasks. In particular, code clone detection can have significant uses in the context of analyzing and fixing bugs in large scale applications. However, prior works, such as machine learning based clone detection, may cause a considerable amount of false positives. In this paper, we propose  {\it Twin-Finder}, a novel, closed-loop approach for pointer-related code clone detection that integrates machine learning and symbolic execution techniques to achieve precision. {\it Twin-Finder} introduces a clone verification mechanism to formally verify if tow clone samples are indeed clones and a feedback loop to automatically generated formal rules to tune machine learning algorithm and further reduce the false positives. Our experimental results show {\it Twin-Finder} the can swiftly identify up 9$\times$ more code clones comparing to conventional code clone detection approaches. We conduct security analysis for memory safety using real-world applications Links version 2.14 and libreOffice-6.0.0.1. {\it Twin-Finder} is able to find 6 unreported bugs in Links version 2.14 and one public patched bug in libreOffice-6.0.0.1. 


 


==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile/.tex/.pdf}; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts
		


==> evaluation.tex <==
\section{Evaluation}
\label{eva}
This section presents a detailed evaluation results of \NAME\ against a tree-based code clone detection tool DECKARD~\cite{jiang2007deckard} in terms of code clone detection, and conduct several case studies for applications security analysis. 
\subsection{Experiment Setup} 
We performed empirical experiments on \NAME. We selected 7 different benchmarks from real-world applications: bzip2, hmmer and sphinx3 from SPEC2006 benchmark suite~\cite{spec}; man and gzip from Bugbench~\cite{lu2005bugbench}; thttpd-2.23beat1~\cite{thttpd_ACME}, a well-known lightweight sever and a lightweight browser links-2.14~\cite{links}.
All experiments are performed on a 2.54 GHz Intel Xeon(R) CPU E5540 8-core server with 12 GByte of main memory. The operating system is ubuntu 14.04 LTS.

To
configure DECKARD, we used the parameter settings proposed by Jiang
et al. ~\cite{jiang2007deckard}, setting minimum token number (minT) as 20, stride to infinite, and code similarity is set between 0.70 and 1.0.


\subsection{Code Clones Detection }
\begin{table}[H]
	\centering

\footnotesize
%	\bgroup
%	\def\arraystretch{1.5}%
%	\resizebox{.48\textwidth}{!}{%
	\begin{tabular}{|c|c|c|c|c|}
		\hline
		\textbf{Bench.} & \textbf{Program Size } & \textbf{\#Code clones} & \textbf{\#Code clones} &\textbf{\% Code clones} \\ 
		& \textbf{(LoC)} & \textbf{without slicing} & \textbf{{Our approach}} &\\ \hline
		\textit{bzip2}     & 5,904                       & 432                            & 1,084         &        150.92\%         \\
		\textit{sphinx3}   & 13,207                      & 1,047                            & 3,546   &         238.68\%          \\
		\textit{hmmer}     & 20,721                      & 1,238                         & 4,391      &          254.68\%           \\
		\textit{thttpd}    & 7,956                       & 611                           & 1,398     &             128.80\%      \\
		\textit{gzip}      & 5,225                       & 36                              & 365        &            913.89\%       \\
		\textit{man}       & 3,028                       & 47                              & 443        &          842.55\%          \\
		\textit{links}     & 178,441                     & 3,007                            & 9,809     &            226.21\%         \\ \hline
	\end{tabular}
%}
%	\egroup
\vspace{0.1in}
\caption{Comparison of number of code clones detected before and after using our approach }
\label{statistics}
\end{table}
\begin{table}[H]
	\centering
\tiny
%		\bgroup
%	\def\arraystretch{1.0}%
%	\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|}
	\hline
	\multirow{2}{*}{\textbf{Bench.}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Pointer related \\ LoC\end{tabular}}} & \multicolumn{2}{c|}{\textbf{Clone Detection w/  DECKARD}} & \multicolumn{2}{c|}{\textbf{Clone Detection w/ Our Approach}} \\ [2ex]\cline{3-6} 
	&                                                                                              & \textbf{\# Cloned LoC}      & \textbf{\% Cloned LoC}      & \textbf{\# D.S LoC}           & \textbf{\% D.S LoC}           \\ \hline
	\textit{bzip2}                      & 3,279                                                                                         & 1,066                        & 32.51\%                     & 2,038                          & 62.15\%                       \\ [2ex]\hline
	\textit{sphinx3}                    & 9,519                                                                                         & 3,073                        & 32.28\%                     & 7,224                          & 75.89\%                       \\ [2ex]\hline
	\textit{hmmer}                      & 11,635                                                                                        & 3,163                        & 27.19\%                     & 6,929                          & 59.55\%                       \\ [2ex]\hline
	\textit{thttpd}                     & 4,390                                                                                         & 1,279                        & 29.13\%                     & 2,267                          & 51.64\%                       \\ [2ex]\hline
	\textit{gzip}                       & 2,289                                                                                         & 219                         & 9.57\%                      & 919                           & 40.15\%                       \\[2ex] \hline
	man                                 & 1,683                                                                                         & 248                         & 14.74\%                     & 826                           & 49.08\%                       \\ [2ex]\hline
	links                               & 28,334                                                                                        & 6,429                        & 22.69\%                     & 18,334                         & 64.71\%                       \\ [2ex]\hline
\end{tabular}
%}
%	\egroup
	\caption{Comparison of code clone coverage between DECKARD and our approach}
	\label{cloned_loc}
\end{table}
We measure code clone quantity by the number of code clones that are detected before and after we use \NAME\ for pointer analysis purpose. We conduct two experiments in terms of the following: code clones quantity, the flexibility of code similarity configuration and false positives analysis.



\begin{figure*}
	\centering

	\subfloat[][thttpd]{\includegraphics[scale=0.2]{clone_plot/thttpd_clone.pdf}\label{<figure6>}}
	\hspace{-0.1in}
	\subfloat[][links]{\includegraphics[scale=0.2]{clone_plot/links_clone.pdf}\label{<figure7>}}
%		\hspace{-0.1in}
	\subfloat[][bzip2]{\includegraphics[scale=0.2]{clone_plot/bzip2_clone.pdf}\label{<figure8>}}
%			\hspace{-0.1in}
	\subfloat[][sphinx3]{\includegraphics[scale=0.2]{clone_plot/sphinx3_clone.pdf}\label{<figure9>}}
				\hspace{-0.1in}
	\subfloat[][hmmer]{\includegraphics[scale=0.2]{clone_plot/hmmer_clone.pdf}\label{<figure10>}}
%					\hspace{-0.1in}
	\subfloat[][man]{\includegraphics[scale=0.2]{clone_plot/man_clone.pdf}\label{<figure11>}}
%						\hspace{-0.1in}
	\subfloat[][gzip]{\includegraphics[scale=0.2]{clone_plot/gzip_clone.pdf}\label{<figure12>}}
	\caption{The amount of code clones detected from \NAME\ with the number of iterations for feedback until converge after relaxing the code similarity from 0.70 to 1.00}
	\label{CodeClones}
\end{figure*}
%\begin{table}[H]
%	\centering
%	
%	
%	\bgroup
%	\def\arraystretch{1.5}%
%	\resizebox{.5\textwidth}{!}{%
%\begin{tabular}{|c|c|c|c|c|c|c|}
%	\hline
%	\multirow{2}{*}{\textbf{Benchmark}} & \multicolumn{3}{c|}{\textbf{\# True Code Clones}}        & \multicolumn{3}{c|}{\textbf{\# Feedback Iterations}}     \\ \cline{2-7} 
%	& \textbf{S = 1.0} & \textbf{S = 0.90} & \textbf{S = 0.80} & \textbf{S = 1.0} & \textbf{S = 0.90} & \textbf{S = 0.80} \\ \hline
%	bzip2                               & 683              & 858               & 1,084             & 1                & 5                 & 10                \\ \hline
%	sphinx3                             & 1,495            & 2,645             & 3,546             & 3                & 10                & 16                \\ \hline
%	hmmer                               & 2,725            & 3,760             & 4,391             & 4                & 12                & 21                \\ \hline
%	man                                 & 102              & 265               & 443               & 1                & 5                 & 12                \\ \hline
%	gzip                                & 66               & 183               & 365               & 1                & 4                 & 11                \\ \hline
%\end{tabular}
%	}
%	\egroup
%	\vspace{0.1in}
%	\caption{Statistics of code clones detected  from \NAME\ with the number of iterations for feedback until converge where S is the code similarity}
%	\label{table:codeclone}
%\end{table}

We evaluated the effectiveness of \NAME\ to show the optimal results \NAME\ are able to achieve. The code similarity is set as 0.80 with feedback enabled to eliminate false positives until converge (no more false positives can be observed or eliminated) in the first experiment. Table~\ref{statistics} shows the size of the corresponding percentage of more code clones detected using our approach. As we can see, the results show that \NAME\ is able to detect 393.68\% more code clones in average compared to the clone detection without slicing and feedback, with the lowest as 128.80\% in \textit{thttpd} and highest up to 913.89\% in \textit{gzip}. Note that our approach achieves the best performance in two smaller benchmark \textit{gzip} and \textit{man}. That is because the number of identical code clones is relatively small in both applications (36 in \textit{gzip} and 47 in \textit{man} respectively). While using our approach, we harness the power of program slicing and feedback using formal analysis, which allows us to detect more true code clones.

Furthermore, we add an additional experiment to address the clone coverage. The goal for clone coverage is, with our optimal configuration, what fraction of a program is detected as cloned code. In this case, we only evaluated the coverage of code clones detected in terms of pointer-related code. We measured the total number of pointer-related code lines cross the entire program and the detected clone lines using DECKARD and our approach as shown in Table~\ref{cloned_loc}. It presents the total detected
pointer related cloned lines, named as \textit{Domain Specific LoC} (D.S LoC), using our approach. The percentage of D.S LoC ranges from 40.15\% to 75.89\%, while for DECKARD the number ranges from 9.57\% to 32.51\%. The results show it is difficult to directly compare the coverage for different applications, because such results are usually sensitive to: (1) the type of application, such as sphinx3 has intensive pointer access, thus it has the highest clone coverage using our approach; (2) the different configurations may lead to different results, since here we set up code similarity as 0.80. However, this experiment is to show that there is a considerable amount of code clones in large code bases in general and our approach can effectively detect such clones and outperforms previous approaches.


In the second experiment, we relaxed the code similarity threshold from 0.70 to 1.00 to show our approach is capable to detect many more code clones within a flexible user-defined configuration. However, it is reasonable to expect more false positives to occur while we are using smaller code similarity. Moreover, we implemented our code clone detection based on DECKARD, which is a syntax tree-based tool and may report semantically
different but syntactically similar code as clones causing more false positives. Note that false negatives
occur if two clone samples have different constraints but are actually the same expression after being solved by the constraint solver. However,
false negatives only result
in actually true clones being missed by \NAME\ and are not critical in security perspective. Thus, we do not evaluate \NAME\ for
false negatives in our study.

To tackle such false positives issue, we enabled a closed-loop feedback to vector embedding as mentioned in the previous section. Thus, we analyzed the effectiveness of our feedback mechanism in terms of eliminating the false positives. 
In this experiment, we applied our feedback as soon as we observed two code clone samples having different constraints obtained from symbolic execution through our clone verification process. We executed several iterations of our feedback until the percentage of false positives converged (no more false positives can be eliminated or observed). Figure~\ref{CodeClones} presents the number of true code clones detected across all the benchmarks from our approach (drawn as red line in each figure) and the number of iterations for feedback needed to converge (shown as the bar plot in each figure) correspondingly. We also repeated the same experiments with three different code similarities setups in other smaller benchmarks. 
%Table~\ref{table:codeclone} shows the results. 
As expected, it takes more iterations for the feedback to converge with smaller code similarity among all benchmarks, and we are still able to detect more true code clones while we reduce the code similarity. However, the results show there is no significant improvement in terms of the number of true code clones increased after code similarity is set as smaller than 0.80. As mentioned in previous section, the code similarity is defined as  $S (T_1, T_2) = \frac{2S}{2S+L+R}$, where $S$ is the number of shared AST nodes in $T_1$ and $T_2$, $L$ and $R$ are the different nodes in two code clone samples. At least 20\% of the AST nodes are different while the code similarity equal to 0.80. 


 
\subsection{Feedback for False Positives Elimination}
\begin{figure}[ht]
	
\centering 
\includegraphics[scale=0.5]{figure/fp_removed.pdf}

\caption{Accumulated percentage of false positives eliminated by \NAME\ with code similarity set to 0.70}
\label{fig:fp_removed}
\end{figure}
We analyzed the number of false positives that could be eliminated by our approach. Here, we chose bzip, thttpd and Links as representative applications to show the results. Figure~\ref{fig:fp_removed} presents the accumulated percentage of false positives eliminated by \NAME\ in each iteration with Code Similarity set to 0.7. Here, we are able to eliminate 99.32\%, 89.0\%, and 86.74\% of false positives in bzip2, thttpd and Links respectively.

The results show our feedback mechanism can effectively remove the majority of false positives admitted from code clone detection. The performance of our feedback is sensitive to different programs due to different program behaviors and program size. As the results show, more feedback iterations are needed for larger program in general (e.g. 26 iterations for bzip2 to converge while 48 iterations for Links, as Links is much larger than bzip2). On the other hand, the number of iterations can also be affected by our clone verification module since we use random sampling approach. Based on the experiment results, we cannot normalize a common removal ratio pattern cross different programs. For instance, 29.83\% of false positives can be eliminated at the first iteration for bzip2, the number is only 13.35\% for thttpd instead. Finally, our feedback may not be able to remove 100\% of false positives, that is because there are several special cases that we cannot remove them using current implementation, such as multiple branches or indirect memory access with the value of array index derived from another pointer. 
\subsection{Bug findings }
\begin{table*}[h]
	\centering
	\tiny
	%	\bgroup
	%	\def\arraystretch{1.5}%
	%	\resizebox{1.0\textwidth}{!}{%
	\begin{tabular}{c|c|c|c|c}

		\hline
		\textbf{Bug Type} & \textbf{Source File}                                                                               & \textbf{Function Name}    & \textbf{Pointer Name}    & \textbf{Bug Report}                                                                                                                                                                                                                           \\ [2ex]\hline

		Null Dereference  & Links-1.4/language.c                                                                               & get\_language\_from\_lang & lang                     & Not Reported           
		 \\ [2ex]\hline

		Null Dereference  & Links-1.4/language.c                                                                               & get\_language\_from\_lang & p                        & Not Reported                                                                                                                                                                                                                                                       \\ [2ex]\hline
		Null Dereference  & Links-1.4/connect.c                                                                                & make\_connection          & host                     & Not Reported            
		\\ [2ex]\hline
		Memory Leak       & Links-1.4/ftp.c                                                                                    & ftp\_logged               & rb                       & Not Reported              
		\\[2ex] \hline
		Memory Leak       & Links-1.4/bfu.c                                                                                    & do\_tab\_compl            & items-\textgreater{}text &Silently patched                                                                                                                                                                                                                                         \\[2ex] \hline
		Memory Leak       & Links-1.4/terminal.c                                                                               & add\_empty\_window        & ewd                      & Not Reported                                                                                                                                                                                                                                                              \\[2ex] \hline
		Buffer Overflow   & \begin{tabular}[c]{@{}l@{}}libreoffice-6.0.0.1/sw/\\source/filter/ww8\\/ww8toolbar.cxx\end{tabular} & SwCTBWrapper::Read        & rCustomizations          & Publicly patched                                                                                                                                                                                        \\[2ex] \hline
	\end{tabular}
	%}
	%\egroup
	\vspace{0.1in}
	\caption{Using our approach to test Links-1.4 and libreoffice-6.0.0.1}
	\label{bugs}
\end{table*}
One benefit of our approach is to use a clone-based approach to enable a rapid security analysis. In this experiment, we use \NAME\ to detect potential vulnerabilities existing in the applications. We use Links version 2.14 and LibreOffice version 6.0.0.1 as representative benchmarks. In particular, we
discovered 6 unique and unreported bugs in Links, including 3 memory leaks and 3 null dereference vulnerabilities. five out of six of the bugs have not been found before, and one of the memory leaks bug has been silently patched in the newer version of Links.

Table~\ref{bugs} shows the
details of these bugs found by our method. Here we show three types of bug examples, null dereference bugs, memory leak and buffer overflow. 
\subsubsection{Links Case Study}


\begin{figure}[h]
\hspace{0.3in}
	\begin{minipage}[b]{0.92\linewidth}
		\begin{lstlisting}[style=CStyle, frame=single,,escapechar=\%]
int get_language_from_lang(unsigned char *lang) {
unsigned char *p;
int i;
%\Hilight%lang = stracpy(lang);
%\Hilight%//Uncheck the memory allocation
%\Hilight%lang[strcspn(cast_const_char lang, ".@")] = 0;
if (!casestrcmp(lang, cast_uchar "nn_NO"))
	strcpy(cast_char lang, "no");
...
search_again;
for (i = 0; i < n_languages(); i++) {
	p = cast_uchar translations[i].t[T__ACCEPT_LANGUAGE].name;
	if (!p)
		continue;
%\Hilight%	p = stracpy(p);
%\Hilight%//Uncheck the memory allocation
%\Hilight%	p[strcspn(cast_const_char p, ",;")] = 0;
	if (!casestrcmp(lang, p)) {
		mem_free(p);
		mem_free(lang);
		return i;
	}
	mem_free(p);
}
...
mem_free(lang);
return -1;
}
\end{lstlisting}
		\caption{Null Dereference bugs in function \textit{get\_language\_from\_lang} of the lightweight browser Links}
				\label{null_dereference}
	\end{minipage}		
\end{figure}
In the first case study, we employ \NAME\ to uncover vulnerabilities in Links, a lightweight browser. The results show \NAME\ finds 6 unreported bugs in Links version 2.14, including 3 memory leaks and 3 Null dereference vulnerabilities. And 1 of the memory leaks bug is silently patched in the newer version of Links. 

%\textbf{First Example}: 
As an example, let us consider the function \textit{get\_language\_from\_lang} shown in Figure~\ref{null_dereference}. This function is implemented as setting language from local serves. This function provides an illustrative example because the programmer confirms that the $stracpy$ requires validation in the comment on
line 5
The $stracpy$ function in line 4 is implemented as dynamic memory allocation for a pointer. The bug arises when the code fails to allocate memory to pointer $lang$ using $stracpy$ function and return $NULL$ to pointer $lang$. Thus, there is a potential null pointer dereference in line 6. 


After we deploy program slicing and code clone detection, we are also able to identify the same bug with the assistance of symbolic execution rapidly for pointer $p$ in line 15, as two code snippets are identified code clones (line 4-6 and line 15-17).
Similarly, pointer $p$ is unchecked after memory allocation, which results in the same vulnerability existing in the codes. This example shows the advantage of our approach combining program slicing and code clone detection for vulnerability discovery.  


%\begin{figure}[ht]
%	
%	
%	
%	\centering 
%	\includegraphics[scale=0.65]{figure/bug2.pdf}
%	\caption{Code snippet from function \textit{Links::ftp\_logged } where a potential memory leak bug via pointer $rb$ is possible}
%	\label{fig:bug_2}
%	
%	%\caption{approach overview}
%\end{figure}
%\begin{figure}[h]
%	\hspace{0.1in}
%\begin{minipage}[b]{0.9\linewidth}
%\begin{lstlisting}[style=CStyle, frame=single,,escapechar=\%]
%static void ftp_logged(struct connection *c)
%{
%struct read_buffer *rb;
%if (!(rb = alloc_read_buffer(c))) return;
%if (!ftp_options.fast_ftp) {
%	ftp_got_user_info(c, rb);
%	return;
%}
%read_from_socket(c, c->sock1, rb, ftp_got_info);
%}
%\end{lstlisting}
%	\caption{Source Code from function \textit{Links::ftp\_logged } where a potential memory leak bug via pointer $rb$ is possible}
%	\label{fig:bug_2}
%\end{minipage}	
%	
%\end{figure}
%\textbf{Second Example}: For the function \textit{Links::ftp\_logged } shown in Figure \ref{fig:bug_2}, \NAME\ reported a potential memory leak vulnerability for pointer $rb$. This function is being used in Links to construct ftp protocol connection and allocate memory space from a local machine. The pointer $rb$ is dynamically allocated memory in line 4 using $alloc\_read\_buffer$ function. Then, it is passed as a function parameter in line 6 and line 9. while \NAME\ deploy symbolic execution, it will look inside both functions in line 6 and line 9. However, the results from symbolic execution show the pointer $rb$ is never freed in either of them. This causes a potential memory leak.
\subsubsection{LibreOffice Case Study}

\begin{figure}[h]
	\hspace{0.3in}
	\begin{minipage}[b]{0.9\linewidth}
		\begin{lstlisting}[style=CStyle, frame=single,,escapechar=\%]
bool SwCTBWrapper::Read( SvStream& rS )
{   
...
if (cCust)
{   
	...
	for (sal_uInt16 index = 0; index < cCust; ++index)
	{   
		Customization aCust( this );
		if ( !aCust.Read( rS ) )
			return false;
		rCustomizations.push_back( aCust );
	}
}
...
std::vector< sal_Int16 >::iterator it_end = dropDownMenuIndices.end();
%\Hilight%for ( std::vector< sal_Int16 >::iterator it = 
%\Hilight%dropDownMenuIndices.begin(); it != it_end; ++it )
{   
%\Hilight%	rCustomizations[ *it ].bIsDroppedMenuTB = true;
}
return rS.good();
}
\end{lstlisting}
\caption{Source Code from function \textit{Links::SwCTBWrapper::Read} where a buffer overflow bug via pointer $rCustomizations$}
\label{fig:bug_3}
	\end{minipage}	
\end{figure}
In the second case study, LibreOffice is an open source office tool, which is written in multiple programming languages including C/C++ and Java. Currently, our approach is working to C/C++ code only. Thus, we only deployed our approach on the C/C++ files in LibreOffice. Our approach was able to identify a heap-based buffer overflow bug in function \textit{Links::SwCTBWrapper::Read}. Figure~\ref{fig:bug_3} shows the original source code. \NAME\ identified a group of code clones of code snippets from line 17-21 in the same cluster. Our feedback mechanism eliminated the other code clones as false positives after 16 iterations.

This function is used to read a crafted document containing a Microsoft Word record (named as a structural array $rCustomizations$ in the source code) from beginning to the end. The size of structural array $rCustomizations$ is defined as $static\_cast<sal\_Int16>( rCustomizations.size() )$. However, the \textit{for} loop in line 17, it does not do a propel bound check of a customizations array index. The value of $*it$ could be negative or larger than the size of  $rCustomizations$. When our approach deploys partial symbolic execution for this $for$ loop, it will yield potential buffer overflow error \footnote{However, after we started our research, this bug has been found earlier of 2018 and public patched in the newer version of LibreOffice. More details about this bug can be found in the report CVE-2018-10120~\cite{libreoffice}}.
%\subsubsection{Speedup}
%We further evaluated the overhead of clone verification using symbolic execution in []  and compared the execution time with
%Pure Symbolic Execution over entire binary programs in terms of bug findings.
%Our baseline is the source code symbolic execution tool KLEE~\cite{cadar2008klee}.
%\begin{table}[h]
%	\centering
%	\bgroup
%	\def\arraystretch{1.2}%
%	\resizebox{0.5\textwidth}{!}{%
%		\begin{tabular}{|c|c|c|}
%			\hline
%			\textbf{\begin{tabular}[c]{@{}c@{}}Pure Symbolic Execution time\\ Function Level (minute)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Symbolic Execution time in \\ {[}{]} (minute)\end{tabular}} & \textbf{Speedup} \\ \hline
%			4119m15s&                                                                                     606m52s     &        6.7$\times$          \\ \hline
%		\end{tabular}
%	}
%	\egroup
%	\caption{Speedup}
%	\label{speedup}
%\end{table}
%
%Table~\ref{speedup} presents the runtime overhead for [] to find all 3 bugs due to pure symbolic execution and []. We evaluate pure symbolic execution overhead and conduct partial symbolic execution on each function as function-level overhead. From previous section, we have observed there is not too much gain on detecting more code clones while the code similarity is smaller than 0.80. Thus, we set up the code similarity as 0.80 in this experiment. Afterwards, we generated total 887 clusters for Links. Note that the smallest cluster contains only 2 code clone samples, we chose a lower bound as 2 code clone samples in our sampling module. For larger clusters, we divide the cluster into three smaller clusters and pick two code samples from each smaller cluster center and boundary respectively and execute a pair wise clone verification process among all the clusters at the same time. The clone verification time spent in [] is calculated as the summation of symbolic execution times in the sampling code clones within each cluster until our feedback to converge, which it took total 27 iterations for feedback (the times spent in sampling are not taken into account).
%
%There are total 2050 out of 2564 functions involving pointer operations from original Links code. To evaluate the function-level symbolic execution overhead, we make use of the symbolic arguments support from KLEE that we make parameters in each function as symbolic data and deploy symbolic execution function by function. Similarly, the pure symbolic execution overhead is the summation of symbolic execution times spent in all 2050 functions. 
%
%
%As we can see, Our approach took 606 minutes while KLEE spent 4119 minutes (around 69 hours) even in function level symbolic execution. The time-to-solution (the time spent to do clone verification and find bugs) for [] is 6
%.7$\times$faster compared to pure symbolic execution in Links.

